LOTUS: Evasive and Resilient Backdoor Attacks through Sub-Partitioning

Backdoor attack poses a significant security threat to Deep Learning applications. Existing attacks are often not evasive to established backdoor detection techniques. This susceptibility primarily stems from the fact that these attacks typically leverage a universal trigger pattern or transformation function, such that the trigger can cause misclassification for any input. In response to this, recent papers have introduced attacks using sample-specific invisible triggers crafted through special transformation functions. While these approaches manage to evade detection to some extent, they reveal vulnerability to existing backdoor mitigation techniques. To address and enhance both evasiveness and resilience, we introduce a novel backdoor attack LOTUS. Specifically, it leverages a secret function to separate samples in the victim class into a set of partitions and applies unique triggers to different partitions. Furthermore, LOTUS incorporates an effective trigger focusing mechanism, ensuring only the trigger corresponding to the partition can induce the backdoor behavior. Extensive experimental results show that LOTUS can achieve high attack success rate across 4 datasets and 7 model structures, and effectively evading 13 backdoor detection and mitigation techniques. The code is available at https://github.com/Megum1/LOTUS.

==> sections/motivation.tex <==
\section{Analysis of Backdoor Uniformity} \label{sec:motivation}

In backdoor attack, an implicit assumption is that the trigger is a secret and difficult to find by defense techniques. However, the current practice of backdoor attack demands that a uniform trigger can flip the classification results of many victim class samples to the target class. We call it
the {\em uniformity} property. Here, a uniform trigger does not mean the trigger has to be a static input pattern. A {\em dynamic trigger} that has various input patterns for different samples may be uniform too, as long as the pattern for an input sample is generated by a uniform  function. For example, in {\em filter attack}, the trigger is injected by applying an Instagram filter to an input. While the filter function is the same, the concrete pixel changes induced by applying the filter vary across inputs.

Uniformity provides strong hints that trigger inversion techniques can leverage to reverse engineer triggers, failing the objective of trigger secrecy. 
Trigger inversion models a trigger as unknown input perturbations~\cite{wang2019neural} or an input transformation function with unknown parameters~\cite{liu2019abs} and then leverages gradient descent to derive valuations of such perturbations/parameters that can flip a set of victim class samples to the target class. The uniformity of existing attacks dictates that the trigger be effective for a large set of samples, providing strong hints to trigger inversion.
Intuitively, one can consider that the trigger flips a given sample as one hint to the identity of trigger.
Uniformity implies that the different victim samples provide a rich set of hints.
Recent results~\cite{shen2021backdoor, sikka2020detecting} from the large scale TrojAI backdoor scanning competition and from scanning advanced backdoors~\cite{liu2021ex} show that trigger inversion is quite effective for identifying various types of backdoor attacks.

Figure~\ref{fig:nc_inverison_patch} shows a ResNet-50 model on ImageNet trojaned with a simple patch trigger~\cite{liu2017trojaning}. Figure (a) shows the victim class ``$Siamese$'' with the injected trigger and (e) shows the target class ``$seashore$''. In (b)-(d), we show the inverted triggers by a popular scanner Neural Cleanse (NC)~\cite{wang2019neural} when 1, 10, and 100 victim samples are used in inversion. Observe that as the number of samples used increases, the inverted triggers change from arbitrary adversarial perturbations to a form exhibiting features of the injected trigger. Note that NC aims to generate the smallest fixed pixel perturbations that
can flip a given set of victim samples to the target class.
Figure~\ref{fig:abs_inverison_patch} shows the results on a VGG-16 model trojaned with a $Gotham$ filter backdoor with (a) an original victim sample and (b) the sample after applying the trigger filer. Note that since the pixel level perturbations are different for various victim samples in filter attack, NC is not effective. However, another scanner ABS~\cite{liu2019abs} can model the trigger as an input transformation function (instead of a fixed pixel pattern) and invert the parameters for the function. Columns 3, 4, and 5 show the victim samples after applying the inverted transformation functions when 1, 10, and 100 samples are used in inversion, respectively. We have similar observations as the patch trigger. That is, when more samples are used in inversion, the resulting trigger has more resemblance to the injected one. More such results for various types of backdoors can be found in Figure~\ref{fig:invert}.
In other words, uniformity indeed leaks trigger identity.

\begin{figure}[ht]
    \begin{minipage}[c]{1\linewidth}
    \subfigure[Injected]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/patch_inject.png}
    \end{minipage}
    }
    \subfigure[Invert 1]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/patch_invert_1.png}
    \end{minipage}
    }
    \subfigure[Invert 10]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/patch_invert_10.png}
    \end{minipage}
    }
    \subfigure[Invert 100]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/patch_invert_100.png}
    \end{minipage}
    }
    \subfigure[Target]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/patch_target.png}
    \end{minipage}
    }
    \caption{NC inversion of a patch trigger.}
    \label{fig:nc_inverison_patch} 
    \end{minipage}
    
    \vspace{7pt}
    
    \begin{minipage}[c]{1\linewidth}
    \subfigure[Victim]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/filter_victim.png}
    \end{minipage}
    }
    \subfigure[Injected]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/filter_inject.png}
    \end{minipage}
    }
    \subfigure[Invert 1]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/filter_invert_1.png}
    \end{minipage}
    }
    \subfigure[Invert 10]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/filter_invert_10.png}
    \end{minipage}
    }
    \subfigure[Invert 100]{
    \begin{minipage}[c]{0.17\linewidth}
        \centering
        \includegraphics[scale=0.2]{figures/filter_invert_100.png}
    \end{minipage}
    }
    \caption{ABS inversion of a filter trigger.}
    \label{fig:abs_inverison_patch}
    \end{minipage}
\end{figure}

\smallskip
\noindent
{\bf Secrecy of Existing Backdoor Attacks.}
In the simplest universal backdoor attack that flips samples of any class to the target class, the secrecy only originates from
the unknown target label because uniformity ensures that as long as the target label is known, there are sufficient hints to support effective trigger inversion.
In general, the scanner has to pick the right target label out of all the possible labels (say $n$).
However, according to K-Arm~\cite{shen2021backdoor}, although the target label is in theory unknown, the current simple data poisoning method (to inject trigger) leaks the target label in many ways. For example, in a trojaned model, although a clean sample is correctly classified, the target label tends to rank high (e.g., top 2 or 3) in the classification result vector; it is in general a lot easier to flip samples to the target label (by small perturbations) compared to flipping to other labels. The bar charts in Figure~\ref{fig:K-arm_rank} show the average ranking of the target label (over a set of samples provided by TrojAI) for 8 trojaned models from TrojAI round 3.
Figure~\ref{fig:K-arm_loss} shows the loss function changes during trigger inversion for all the labels in a trojaned model \#84 from TrojAI round 3 with the target label 0. Observe that the loss value has the steepest drop for the target label (i.e., it is the easiest to optimize). This supports that the practical secrecy is much lower than guessing 1 out of $n$ for universal attacks. The same observations hold for label-specific attacks, whose practical secrecy is much lower than guessing 1 out of the $n\times(n-1)$ pairs of victim-target labels.
It explains the effectiveness of existing trigger inversion based scanners.

\begin{figure}
    \begin{minipage}[c]{0.48\columnwidth}
        \centering
        \includegraphics[width=1.7in]{figures/K-arm_rank.png}
        \caption{Average ranking of target label}
        \label{fig:K-arm_rank}
    \end{minipage}
    ~
    \begin{minipage}[c]{0.48\columnwidth}
        \centering
        \includegraphics[width=1.7in]{figures/K-arm_loss.png}
        \caption{Loss changes during trigger inversion}
        \label{fig:K-arm_loss}
    \end{minipage}
\end{figure}



\smallskip
\noindent
{\bf Breaking Uniformity.}
We observe that the uniformity property is not essential to backdoor attack. The overarching idea of our method is hence to suppress uniformity such that trigger secrecy can be substantially escalated.
Specifically, we use a partitioning function to separate all the samples in the victim class to $m$ partitions and poison each partition with a unique trigger. The partitioning function and the $m$ different triggers become the secret
of the attacker. To launch attack with a test input, the attacker applies the partitioning function to the input to determine which of the $m$ partitions it belongs to and then stamps the corresponding trigger. The perturbed input hence induces the misclassification to the target label. The key insight is that {\em a random set of victim samples are likely not from the same partition such that using them in trigger inversion would provide contradicting hints to the optimizer. As a result, the trigger(s) cannot be properly inverted.} Furthermore, even if the set of victim samples by chance belong to a partition, one inverted trigger is not sufficient to induce a high attack success rate for other images because different triggers are needed to attack different partitions. As a result, scanners likely concludes that the model is clean.

Figure~\ref{fig:NEEDLE_inverted_triggers:a} shows samples from four partitions of the ``$bird$'' class in a VGG-16 model on ImageNet with the corresponding triggers.
Figure~\ref{fig:NEEDLE_inverted_triggers}(b-e) show the inversion results using NC with different assumptions.
Figure~\ref{fig:NEEDLE_inverted_triggers:b} shows the inversion results when we assume the precise partitions are known to the scanner. That is, we invert four triggers for the four partitions separately and use 100 samples from each partition. Observe that the inverted triggers contain features of the injected ones. More importantly, they are quite small (with average size 372.8), much smaller than the inverted triggers for labels that are not compromised. 
Such size differences are leveraged by existing scanners such as NC, ABS, and K-Arm to detect backdoor.
In contrast, Figure~\ref{fig:NEEDLE_inverted_triggers:c} shows the inverted trigger when an arbitrary set of 100 samples (from all four partitions) are used. Observe that the trigger is much larger with the size of 1025.9, which is not distinguishable from inverted triggers between clean labels.
As such, the scanner fails to detect the backdoor. Figure~\ref{fig:NEEDLE_inverted_triggers:d} shows the inverted results (of two partitions) when we assume the partition number is known by the scanner and the scanner guesses half of the samples' partitions correct.
In other words, we use four different subsets of victim class samples to invert four respective triggers and each subset has half of the samples belonging to the same partition. Observe that even with such a strong assumption, the triggers are still very large, failing the detection.
Figure~\ref{fig:NEEDLE_inverted_triggers:e} shows the inverted results when four individual samples from the four respective partitions are used. Observe that the inverted triggers are small perturbations that are not uniform at all. The reason is that flipping the classification of one sample is easy, like in adversarial attack. The generated  triggers are essentially small adversarial perturbations and likely do not possess substantial trigger features.




\iffalse
\smallskip
\noindent
{\em Key Challenge.} Simple data poisoning is insufficient for our attack. Specifically, stamping the $m$ triggers on samples of the $m$ partitions and setting the classification results to the target label does not work well. The reason is that 
data poisoning cannot effectively bound the scope of a partition trigger such that the trigger likely flips samples in other partitions. According to our results in Section~\ref{sec:valid_adv}, a trigger can achieve a high attack success rate (ASR) (over 95\%) for all partitions if simple poisoning is used. Intuitively, although we separate the victim class to many partitions, these partitions nonetheless share a lot of common features (as they belong to the same class) and consequently poisoning one partition may have substantial effects on other partitions as well. This is problematic as it suggests uniformity, allowing easy detection. In Section~\ref{sec:triggerfocus}, we propose a new training method called {\em trigger focusing} that ensures a trigger is only effective for its own partition.
\fi



\begin{figure}[t]
\centering
    \subfigure[\label{fig:NEEDLE_inverted_triggers:a} Original injected trigger patterns]{
    \begin{minipage}[c]{1.0\linewidth}
        \centering
        \includegraphics[width=0.75in]{figures/nc_sample_0.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_sample_1.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_sample_2.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_sample_3.png}
    \end{minipage}
    }
    
    \subfigure[\label{fig:NEEDLE_inverted_triggers:b} Inverted trigger patterns given 4 correct partitions]{
    \begin{minipage}[c]{1.0\linewidth}
        \centering
        \includegraphics[width=0.75in]{figures/nc_fusion_0_size.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_fusion_1_size.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_fusion_2_size.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_fusion_3_size.png}
    \end{minipage}
    }
    
    \hspace{6pt}
    \subfigure[\label{fig:NEEDLE_inverted_triggers:c} No partition]{
    \begin{minipage}[c]{0.25\linewidth}
        \centering
        \includegraphics[width=0.75in]{figures/nc_fusion_0123_size.png}
    \end{minipage}
    }
    \subfigure[\label{fig:NEEDLE_inverted_triggers:d} Half correct partitions]{
    \hspace{3pt}
    \begin{minipage}[c]{0.5\linewidth}
        \centering
        \includegraphics[width=0.75in]{figures/nc_fusion_20_size.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_fusion_31_size.png}
    \end{minipage}
    \hspace{5pt}
    }
    
    \subfigure[\label{fig:NEEDLE_inverted_triggers:e} Inverted trigger patterns given a single sample from each partition]{
    \begin{minipage}[c]{1.0\linewidth}
        \centering
        \includegraphics[width=0.75in]{figures/nc_per_fusion_0_size.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_per_fusion_1_size.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_per_fusion_2_size.png}
        \hspace{2pt}
        \includegraphics[width=0.75in]{figures/nc_per_fusion_3_size.png}
    \end{minipage}
    }
    
    \caption{\sname{} attacking the ``{\em bird}'' class of a model on ImageNet and the inverted samples with various assumptions. The number on each inverted trigger denotes its size.}
    \label{fig:NEEDLE_inverted_triggers}
\end{figure}

